Structuring Latent Spaces for Stylized Response Generation

Generating responses in a targeted style is a useful yet challenging task, especially in the absence of parallel data. With limited data, existing methods tend to generate responses that are either less stylized or less context-relevant. We propose StyleFusion, which bridges conversation modeling and non-parallel style transfer by sharing a structured latent space. This structure allows the system to generate stylized relevant responses by sampling in the neighborhood of the conversation model prediction, and continuously control the style level. We demonstrate this method using dialogues from Reddit data and two sets of sentences with distinct styles (arXiv and Sherlock Holmes novels). Automatic and human evaluation show that, without sacrificing appropriateness, the system generates responses of the targeted style and outperforms competitive baselines.

==> sections/table_vs_r.tex <==


\begin{table}[h]
    \centering
    \small
    \begin{tabular}{p{0.07\textwidth}|p{0.36\textwidth}} \hline 
    \textbf{context} & Okay, but can we host it in the cloud?\\
    \hline
    $\rho=0.3$ & Yes.\\
    $\rho=0.5$ & I would like to know this as well. \\
    $\rho=1.0$ & It would be an interesting experiment. It is a possibility. \\
    \hline
    \textbf{context} & The universe has no edge.\\
    \hline
    $\rho=0.0$ & I think that was the point.\\
    $\rho=0.6$ & The universe is infinite  \\
    $\rho=1.0$ & Does this mean the universe is expanding? \\
    \hline
    \end{tabular}
    \caption{Example \textsc{StyleFusion} outputs for arXiv-like response generation task}
    \label{table:example_arXiv}
\end{table}

\begin{table}[h]
    \centering
    \small
    \begin{tabular}{p{0.07\textwidth}|p{0.36\textwidth}} \hline 
    \textbf{context} & First step: go check behind the cabinet and see what's back there.\\
    \hline
    $\rho=0.0$ & I'm going to go ahead and say this. \\
    $\rho=0.6$ & I have a feeling that will be the case.\\
    $\rho=1.0$ & I would advise against this. \\
    \hline
    \textbf{context} & That's a surprisingly large amount of police coming to see a *** teenager\\
    \hline
    $\rho=0.2$ & I'm not sure if you 're serious .\\
    $\rho=0.3$ & I'm going to go ahead and say that it 's not a bad idea .  \\
    $\rho=1.0$ & What is this crime you speak of? \\
    \hline
    \end{tabular}
    \caption{Example \textsc{StyleFusion} outputs for Holmes-like response generation task}
    \label{table:example_holmes}
\end{table}

